Axion Dark Matter Research with IBS/CAPP

The axion, a consequence of the PQ mechanism, has been considered as the most elegant solution to the strong-CP problem and a compelling candidate for cold dark matter. The Center for Axion and Precision Physics Research (CAPP) of the Institute for Basic Science (IBS) was established on 16 October 2013 with a main objective to launch state of the art axion experiments in South Korea. Relying on the haloscope technique, our strategy is to run several experiments in parallel to explore a wide range of axion masses with sensitivities better than the QCD axion models. We utilize not only the advanced technologies, such as high-field large-volume superconducting (SC) magnets, ultra low temperature dilution refrigerators, and nearly quantum-limited noise amplifiers, but also some unique features solely developed at the Center, including high-quality SC resonant cavities surviving high magnetic fields and efficient cavity geometries to reach high-frequency regions. Our goal is to probe axion dark matter in the frequency range of 1-10 GHz in the first phase and then ultimately up to 25 GHz, even in a scenario where axions constitute only 10% of the local dark matter halo. In this report, the current status and future prospects of the experiments and R&D activities at IBS/CAPP are described.

==> 1.3.5/main.tex <==
\subsection{18\,T HTS magnet}
18\,T magnet dimension is particularly designed to probe axion mass range of 14\,$\mu$eV and 18\,$\mu$eV at KSVZ axion model range. An experiment to detect very tiny signal (10$^{- 24}\,$W) in a very strong magnetic field (18\,T) at an ultra-low temperature (300\,mK) has never been performed before, hence it is the most sensitive dark matter axion search experiment on the planet in the corresponding mass range. The dimension of the magnet has been determined in order to pursue the potential physics outcomes by probing a number of interesting axion masses predicted by theoretical models in cosmology. 

Low temperate superconductor magnet can produce magnetic field only in the liquid helium (4.2\,K). Current density of HTS is higher than LTS, moreover Ic properties of HTS in magnetic field is better. Thus very high field magnet must need HTS conductor. However, critical problem of very strong magnetic field magnet is soft insulation material. Strong Lorenz force can destroy insulator in the HTS magnet. Thus no insulation magnet technic is developed and successfully demonstrated.  

Recently, no insulation small magnet produces magnetic field up to 45\,T (NHMFL, USA). Successfully developed 26\,T, 35\,mm magnet by SuNAM, Korea. Most impressive advantage of no insulation magnet is protecting itself from quench without any other protection system. Insulation type magnet can be damaged by quench because of thermal run away, so it must have quench protection system. However, current of no insulation magnet can pass through turn to turn when quench occurs. So, large bore, high field no-insulation magnet is developing world wide.  

18\,T HTS magnet which has 70\,mm bore size was developed by SuNAM from 2016. No insulation technique was applied to the developing 18\,T magnet. 
Critical current of HTS coil is affected by magnitude of magnetic field. Generally, critical current decreeing by magnetic field. Strongest magnetic field on superconductor surface appears top and bottom coil. Thus, critical current at top and bottom are minimum and it decides operating current of whole magnet system. Wider coil has much more critical current thus multi width magnet design is profitable to maximize operating current. Multi width double pancake coils were used to designing 18\,T magnet, 4$-$12\,mm width superconductor tapes were used for manufacturing magnet. Developed magnet system was delivered, installed and tested at CAPP in August 2017.
Figure~\ref{fig:CAPP-18T-1} shows the magnetic field analysis results of 18\,T magnet and Fig.~\ref{fig:CAPP-18T-2} is actual magnet system which is delivered to CAPP.

\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{1.3.5/figures/18T_FEM}
\caption{\label{fig:CAPP-18T-1}FEM analysis of 18\,T HTS magnet}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{1.3.5/figures/18T_install}
\caption{\label{fig:CAPP-18T-2}Installation of 18\,T HTS magnet at CAPP in 2017, Aug.}
\end{figure}

%\begin{figure}[h]
%\centering
%\includegraphics[width=0.8\textwidth]{1.3.5/figures/18T_initial_cooling}
%\caption{\label{fig:CAPP-18T-3}Initial cooling for 18\,T magnet experiment}
%\end{figure}

\begin{table}
\centering
\caption{\label{tab:1}Specifications of 18\,T magnet system}
\begin{tabular}{cc}
\hline
Specifications & Value \\
\hline
Magnet length & 522\,mm \\
Bore diameter & 70\,mm \\
Superconductor & GdBCO, Sunam\\
Conductor width & 4~12\,mm (multi width)\\
Operating temperature & 4.2 K\\
Center magnetic field & 18\,T @ 199.2 A\\
Helium consumption & 114 L/day\\
\hline
\end{tabular}
\end{table}

Inner diameter and total length of the magnet are 70\,mm, 600\,mm respectively. Magnet was installed in the cryostat which has liquid nitrogen and vacuum jacket outside to minimize heat invasion into magnet system. It helps saving liquid helium consumption. After filling liquid helium in the cryostat, current applied to the magnet using power supply. When current is ramping up, induced current generates additional heat thus current lamped up with several steps. Current ramping up rate was 0.02\,A/s to 180\,A than, ramping rate is slow down 0.01\,A/s to 199.2\,A. Current charging time is 6 hours to 199.2\,A however, magnetic field is not proportional to current directly because this magnet does not have insulation between conductor. So, to get the 18\,T magnetic field, it takes 2 more hours after current ramping up. During the magnet charging, helium consumption rate is increasing due to induced current. 

Magnetic field of 18\,T magnet was measured using hall sensors from top to bottom. Figure~\ref{fig:CAPP-18T-4} shows the magnetic field profile on z-axis of the magnet. Uniformity of center magnetic field at $\pm$ 100\,mm is 93\% of center field and magnetic field at the end of magnet was 8\,T. 

\begin{figure}[b]
\centering
\includegraphics[width=0.9\textwidth]{1.3.5/figures/Field_mapping}
\caption{\label{fig:CAPP-18T-4}Magnetic field mapping results.}
\end{figure}

Figure~\ref{fig:CAPP-18T-5} shows the detail ramping up characteristic of 18\,T magnet. Current ramping up was divided 4 steps up to 199.2\,A for 18\,T magnetic field. Because strong stress affected to magnet structure and eddy current generates more heat in the magnet. Current ramping up rates are 0.02\,A/s (1.2\,A/min) up to 150 A, 0.01\,A/s (0.6 A/min) up to 199.2\,A respectively. After charging voltage of the magnet is 9.2\,mV because of copper connections and joint resistance between 44 DPCs. Calculated electrical heat load is 1.83\,W. Total heat load can be estimated from helium consumption rate. Helium consumption rate was measured at steady state of magnet system and 2.83 liters of liquid helium consumed hourly. Thus total teat load of 18\,T HTS magnet, cryostat, and all system as shown in Fig~\ref{fig:CAPP-18T-6}. is 3.96\,W and 67.92 liters of liquid helium requires daily. Considering helium transfer losses, 112 liters of liquid helium requires. Additional heat load may added to the system if cavity and dilution system are installed in the magnet system.

\begin{figure}[h]
\centering
\includegraphics[width=0.9\textwidth]{1.3.5/figures/Magnet_charging}
\caption{\label{fig:CAPP-18T-5}Magnet charging characteristic.}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=1.0\textwidth]{1.3.5/figures/Cryostat_test}
\caption{\label{fig:CAPP-18T-6}Cryostat performance test results}
\end{figure}

For long time experiment, stable liquid helium supply is most important works. Liquid helium is refilling manually however, it must refill every 15 hours during experiment. Thus, we developed automatic helium refilling system for stable operation of magnet system. Figure~\ref{fig:CAPP-18T-7} shows the conceptual design of automatic refilling system and Fig.~\ref{fig:CAPP-18T-8} is developed system. Monitoring and control system was developed using Labview and DAQ system. 

Control system monitoring liquid helium level and it controls pressure of liquid helium Dewar to filling liquid helium. We tested over 2 weeks with automatic refilling system and it was stable to keep operating condition. Two of liquid helium Dewar was consumed weekly, total 2000 liters of liquid helium consumed for long time operation test. 52,000 liters of liquid helium requires for one year operation. Total running cost is 0.52 billion KRW (2018, 14000 KRW/liter, ). It depends on operating condition.

\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{1.3.5/figures/Helium_refilling}
\caption{\label{fig:CAPP-18T-7}Configuration of automatic helium refilling system}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{1.3.5/figures/Helium_refilling_with18T}
\caption{\label{fig:CAPP-18T-8}Automatic liquid helium refilling system with 18\,T HTS magnet at CAPP}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{1.3.5/figures/Helium_refilling_test}
\caption{\label{fig:CAPP-18T-9}Long time test (2 weeks) results with automatic control system}
\end{figure}

\subsection{Cavity installation}
RF-cavity was installed at 18\,T magnet system. Figure~\ref{fig:CAPP-18T-10} shows the installed cavity, amplifiers and tuning rod control system. Tuning rod control system designed for low temperature operation. Two step motors controlling tuning rod and RF antenna position. Low temperature noise level of amplifiers were measured in 18\,T field.

\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{1.3.5/figures/Cavity_install}
\caption{\label{fig:CAPP-18T-10}RF cavity installation for axion search}
\end{figure}

Table~\ref{tab:2}. shows test summary of 18\,T magnet at CAPP. We have done HTS magnet performance verification, noise test of RF cavity and tuning mechanism test. Now we are preparing dilution refrigerator and axion experiment will start soon.

\begin{table}[h]
\centering
\caption{\label{tab:2}18\,T magnet test summary}
\begin{tabular}{lllll}
\hline
Test & date & Purpose & \makecell{Max current\\ and B field} & \makecell{Operation\\ time} \\
\hline
1\textsuperscript{st}  & 2017/8/28 & Inspection & 207 A / 18.7 T & 2 hours \\
2\textsuperscript{nd} & 8/30 & First operation & 207 A / 18.7 T & 2 days \\
3\textsuperscript{rd}  & 10/30 & Long time stability test & 199.2 A / 18\,T & 2 weeks \\
4\textsuperscript{th}  & 2018/1/25 & Cavity install & 199.2 A / 18\,T & 2 days \\
5\textsuperscript{th}  & 2/14 & Field mapping  & 199.2 A / 18\,T & 1 day \\
6\textsuperscript{th} & 3/12 & Cavity test & 199.2 A / 18\,T & 1 week \\
7\textsuperscript{th}  & 4/11 & Cavity test & 199.2 A / 18\,T & 3 days \\
8\textsuperscript{th} & 5/30 & Cavity test & 199.2 A / 18\,T & 3 days \\
\hline
\end{tabular}
\end{table}

